Automatic Generation of Complete Polynomial Interpolation Hardware Design Space

Hardware implementations of complex functions regularly deploy piecewise polynomial approximations. This work determines the complete design space of piecewise polynomial approximations meeting a given accuracy specification. Knowledge of this design space determines the minimum number of regions required to approximate the function accurately enough and facilitates the generation of optimized hardware which is competitive against the state of the art. Targeting alternative hardware technologies simply requires a modified decision procedure to explore the space.

==> dse_procedures.tex <==
\begin{tikzpicture}

\node [shape=rectangle,draw = black, minimum width = 1cm] at (2,3) (min_k_lut_crit) {Min $k$};

% Square Crit DSE Method
\node at (0.2,2.7) {Square Crit};
\node [shape=rectangle,draw = black, minimum width = 1cm, fill=red!20]   at (0,2) (sq_trunc_sq_crit) {Max square trunc};
\node [shape=rectangle,draw = black, minimum width = 1cm, fill=blue!20]  at (0,1) (lin_trunc_sq_crit) {Max linear trunc};
\node [shape=rectangle,draw = black, minimum width = 1cm, fill=green!20] at (0,0) (a_prec) {Min $a$ bitwidth};
\node [shape=rectangle,draw = black, minimum width = 1cm, fill=green!20] at (0,-1) (b_prec) {Min $b$ bitwidth};
\node [shape=rectangle,draw = black, minimum width = 1cm, fill=green!20] at (0,-2) (c_prec) {Min $c$ bitwidth};

\draw [->,very thick] (min_k_lut_crit) edge (sq_trunc_sq_crit);
\draw [->,very thick] (sq_trunc_sq_crit) edge (lin_trunc_sq_crit);
\draw [->,very thick] (lin_trunc_sq_crit) edge (a_prec);
\draw [->,very thick] (a_prec) edge (b_prec);
\draw [->,very thick] (b_prec) edge (c_prec);

% LUT Crit DSE Method
% \node at (3.8,2.7) {LUT Crit};
% \node [shape=rectangle,draw = black, minimum width = 1cm, fill=green!20] at (4,2) (lut_width) {Min LUT width};
% \node [shape=rectangle,draw = black, minimum width = 1cm, fill=red!20]   at (4,1) (sq_trunc_lut_crit) {Max square trunc};
% \node [shape=rectangle,draw = black, minimum width = 1cm, fill=blue!20]  at (4,0) (lin_trunc_lut_crit) {Max linear trunc};

% \draw [->,very thick] (min_k_lut_crit) edge (lut_width);
% \draw [->,very thick] (lut_width) edge (sq_trunc_lut_crit);
% \draw [->,very thick] (sq_trunc_lut_crit) edge (lin_trunc_lut_crit);


\end{tikzpicture}
